Geometric Bounds on the Fastest Mixing Markov Chain

In the Fastest Mixing Markov Chain problem, we are given a graph $G = (V, E)$ and desire the discrete-time Markov chain with smallest mixing time $\tau$ subject to having equilibrium distribution uniform on $V$ and non-zero transition probabilities only across edges of the graph. It is well-known that the mixing time $\tau_\textsf{RW}$ of the lazy random walk on $G$ is characterised by the edge conductance $\Phi$ of $G$ via Cheeger's inequality: $\Phi^{-1} \lesssim \tau_\textsf{RW} \lesssim \Phi^{-2} \log |V|$. Analogously, we characterise the fastest mixing time $\tau^\star$ via a Cheeger-type inequality but for a different geometric quantity, namely the vertex conductance $\Psi$ of $G$: $\Psi^{-1} \lesssim \tau^\star \lesssim \Psi^{-2} (\log |V|)^2$. This characterisation forbids fast mixing for graphs with small vertex conductance. To bypass this fundamental barrier, we consider Markov chains on $G$ with equilibrium distribution which need not be uniform, but rather only $\varepsilon$-close to uniform in total variation. We show that it is always possible to construct such a chain with mixing time $\tau \lesssim \varepsilon^{-1} (\operatorname{diam} G)^2 \log |V|$. Finally, we discuss analogous questions for continuous-time and time-inhomogeneous chains.

==> FMMC_Sections/FMMC_Introduction/FMMC_Structure.tex <==
Maybe we should include a ``structure of the paper'' section?


==> FMMC_Sections/FMMC_Misc.tex <==
\color{blue}
Possible open problems:
\begin{enumerate}
\item Cheeger-type inequality for arbitrary stationary distributions
\item Minor open problem: we have a $\log n$ factor in the Cheeger-type result, but the SSE conjecture 
	would allow having a $\log \dmax$ factor instead.
\item Possible applications of our results? For example, 
	is it possible to use the insights from almost-mixing to design faster ``practical''
	chains for some applications?
\item convoluted open problem: is it possible to sparsify a graph so that the resulting graph has only
	$O(n)$ edges but has vertex-conductance of the same order as the original graph?
	By our results and sparsification results in the literature, we can obtain a sparsifier which has vertex conductance
	at least $\VC^2/{\log n}$.
\end{enumerate}

\color{black}
